Modelling publication bias and p-hacking

Publication bias and p-hacking are two well-known phenomena that strongly affect the scientific literature and cause severe problems in meta-analyses. Due to these phenomena, the assumptions of meta-analyses are seriously violated and the results of the studies cannot be trusted. While publication bias is almost perfectly captured by the weighting function selection model, p-hacking is much harder to model and no definitive solution has been found yet. In this paper we propose to model both publication bias and p-hacking with selection models. We derive some properties for these models, and we compare them formally and through simulations. Finally, two real data examples are used to show how the models work in practice.

==> figures/phacking_type_i.tex <==
\tikz{
	
	% nodes
	\node[obs] (xstar) {$x$};%
	\node[latent, above=of xstar] (thetastar) {$\theta$};%
	\node[latent, above=of thetastar, xshift = -1cm, yshift = .5cm] (theta0) {$\theta_0$}; %
	\node[const, left=of xstar] (sigma) {$\sigma$}; %
	\node[latent, above=of thetastar, xshift = 1cm, yshift = .5cm] (tau) {$\tau$}; %
	\node[obs, below=of xstar] (u) {$u$}; %
	\node[latent, right=of thetastar] (Z) {$Z$}; %
	
	% plates
	\plate [inner sep = .5cm, dashed]
	  {selection} 
	  {(thetastar)(xstar)(u)} 
	  {}; 
	
	\plate [inner sep = .5cm] 
	  {sampling} 
	  {(sigma)(thetastar)(xstar)(selection)(u)(Z)} 
	  {};
	
	% edges
	\edge {theta0,tau} {thetastar} 
	\edge {thetastar,sigma} {xstar} 
	\edge {sigma, xstar} {u}
	\edge {u,Z} {selection} 
}


==> figures/phacking_type_ii_-_Copy.tex <==
\tikz{
	
	% nodes
	\node[obs] (xstar) {$x$};%
	\node[latent, above=of xstar] (thetastar) {$\theta$};%
	\node[latent, above=of thetastar, xshift = -1cm, yshift = .5cm] (theta0) {$\theta_0$}; %
	\node[const, left=of xstar] (sigma) {$\sigma$}; %
	\node[latent, above=of thetastar, xshift = 1cm, yshift = .5cm] (tau) {$\tau$}; %
	\node[obs, below=of xstar] (u) {$u$}; %
	\node[latent, right=of thetastar] (Z) {$Z$}; %
	
	% plates
	\plate [inner sep = .5cm, dashed]
	{selection} 
	{(xstar)(u)} 
	{}; 
	
	\plate [inner sep = .5cm] 
	{sampling} 
	{(sigma)(thetastar)(xstar)(selection)(u)(Z)} 
	{};
	
	% edges
	\edge {theta0,tau} {thetastar} 
	\edge {thetastar,sigma} {xstar} 
	\edge {sigma, xstar} {u}
	\edge {u,Z} {selection} 
}


==> figures/publication_bias_type_i_-_Copy.tex <==
\tikz{
	
	% nodes
	\node[obs] (xstar) {$x$};%
	\node[latent, above=of xstar] (thetastar) {$\theta$};%
	\node[latent, above=of thetastar, xshift = -1cm, yshift = .5cm] (theta0) {$\theta_0$}; %
	\node[const, left=of xstar] (sigma) {$\sigma$}; %
	\node[latent, above=of thetastar, xshift = 1cm, yshift = .5cm] (tau) {$\tau$}; %
	\node[latent, above=of thetastar, yshift = .5cm] (rho) {$\rho$};
	\node[obs, below=of xstar] (u) {$u$}; %
	
	% plates
	\plate [inner sep = .5cm, dashed]
	{selection} 
	{(thetastar)(xstar)(u)} 
	{}; 
	
	\plate [inner sep = .5cm] 
	{sampling} 
	{(sigma)(thetastar)(xstar)(selection)(u)} 
	{};
	
	% edges
	\edge {theta0,tau} {thetastar} 
	\edge {thetastar,sigma} {xstar} 
	\edge {sigma, xstar} {u}
	\edge {u, rho} {selection} 
}



==> figures/publication_bias_type_ii.tex <==
\tikz{
	
	% nodes
	\node[obs] (xstar) {$x$};%
	\node[latent, above=of xstar] (thetastar) {$\theta$};%
	\node[latent, above=of thetastar, xshift = -1cm, yshift = .5cm] (theta0) {$\theta_0$}; %
	\node[const, left=of xstar] (sigma) {$\sigma$}; %
	\node[latent, above=of thetastar, xshift = 1cm, yshift = .5cm] (tau) {$\tau$}; %
	\node[obs, below=of xstar] (u) {$u$}; %
	
	% plates
	\plate [inner sep = .5cm, dashed]
	{selection} 
	{(xstar)(u)} 
	{}; 
	
	\plate [inner sep = .5cm] 
	{sampling} 
	{(sigma)(thetastar)(xstar)(selection)(u)} 
	{};
	
	% edges
	\edge {theta0,tau} {thetastar} 
	\edge {thetastar,sigma} {xstar} 
	\edge {sigma, xstar} {u}
	\edge {u} {selection} 
}



==> figures/simple_example_3.tex <==
\tikz{
	
	% nodes
	\node[obs] (s) {$s$};%
	\node[obs, above=of s] (x) {$x$};%
	\node[obs, above=of x] (theta) {$\theta$}; %
	
	% plates
	\plate [inner sep = .5cm, dashed]
	{selection} 
	{(theta)} 
	{}; 
	
	
	% edges
	\edge {theta} {x} 
	\edge {x} {s} 
	
}

==> figures/underlying_model.tex <==

	\tikz{
		% nodes
		\node[obs] (xstar) {$x$};%
		\node[latent, above=of xstar] (thetastar) {$\theta$};%
		\node[latent, above=of thetastar, xshift = 1cm] (tau) {$\tau$}; %
		\node[latent, above=of thetastar, xshift = -1cm] (theta0) {$\theta_0$}; %
		\node[const, left=of xstar] (sigma) {$\sigma$}; %
		% plate
		\plate [inner sep = .5cm]  
		    {sampling} 
		    {(sigma)(thetastar)(xstar)} 
		    {}; 
		% edges
		\edge {theta0, tau} {thetastar} 
		\edge {thetastar, sigma} {xstar} 
	}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

